Occupancy Networks: Learning 3D Reconstruction in Function Space

With the advent of deep neural networks, learning-based approaches for 3D reconstruction have gained popularity. However, unlike for images, in 3D there is no canonical representation which is both computationally and memory efficient yet allows for representing high-resolution geometry of arbitrary topology. Many of the state-of-the-art learning-based 3D reconstruction approaches can hence only represent very coarse 3D geometry or are limited to a restricted domain. In this paper, we propose Occupancy Networks, a new representation for learning-based 3D reconstruction methods. Occupancy networks implicitly represent the 3D surface as the continuous decision boundary of a deep neural network classifier. In contrast to existing approaches, our representation encodes a description of the 3D output at infinite resolution without excessive memory footprint. We validate that our representation can efficiently encode 3D structure and can be inferred from various kinds of input. Our experiments demonstrate competitive results, both qualitatively and quantitatively, for the challenging tasks of 3D reconstruction from single images, noisy point clouds and coarse discrete voxel grids. We believe that occupancy networks will become a useful tool in a wide variety of learning-based 3D tasks.

==> tables/table_img2mesh_small.tex <==
\begin{tabular}{lccc}
\toprule
{} &             IoU &   Chamfer-$L_1$ & Normal Consistency \\
\midrule
3D-R2N2  &           0.493 &           0.278 &              0.695 \\
PSGN     &               - &           0.215 &                  - \\
Pix2Mesh &           0.480 &           0.216 &              0.772 \\
AtlasNet &               - &  \textbf{0.175} &              0.811 \\
ONet     &  \textbf{0.571} &           0.215 &     \textbf{0.834} \\
\bottomrule
\end{tabular}


==> tables/table_onet_psgn.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
{} & \multicolumn{3}{c}{IoU} & \multicolumn{3}{c}{Chamfer-$L_1$} & \multicolumn{3}{c}{Normal Consistency} \\
{} & PSGN &            ONet &     ONet + PSGN &            PSGN &            ONet &     ONet + PSGN &               PSGN &            ONet &     ONet + PSGN \\
category    &      &                 &                 &                 &                 &                 &                    &                 &                 \\
\midrule
airplane    &    - &           0.571 &  \textbf{0.598} &           0.137 &           0.147 &  \textbf{0.119} &                  - &           0.840 &  \textbf{0.854} \\
bench       &    - &  \textbf{0.485} &           0.438 &           0.181 &           0.155 &  \textbf{0.152} &                  - &  \textbf{0.813} &           0.791 \\
cabinet     &    - &  \textbf{0.733} &           0.711 &           0.215 &           0.167 &  \textbf{0.166} &                  - &  \textbf{0.879} &           0.869 \\
car         &    - &  \textbf{0.737} &           0.723 &           0.169 &           0.159 &  \textbf{0.151} &                  - &  \textbf{0.852} &           0.838 \\
chair       &    - &  \textbf{0.501} &           0.498 &           0.247 &           0.228 &  \textbf{0.207} &                  - &  \textbf{0.823} &           0.813 \\
display     &    - &           0.471 &  \textbf{0.507} &           0.284 &           0.278 &  \textbf{0.248} &                  - &  \textbf{0.854} &  \textbf{0.854} \\
lamp        &    - &  \textbf{0.371} &           0.364 &           0.314 &           0.479 &  \textbf{0.305} &                  - &           0.731 &  \textbf{0.741} \\
loudspeaker &    - &  \textbf{0.647} &           0.637 &           0.316 &           0.300 &  \textbf{0.284} &                  - &  \textbf{0.832} &           0.824 \\
rifle       &    - &           0.474 &  \textbf{0.481} &  \textbf{0.134} &           0.141 &           0.135 &                  - &           0.766 &  \textbf{0.778} \\
sofa        &    - &  \textbf{0.680} &           0.673 &           0.224 &           0.194 &  \textbf{0.188} &                  - &  \textbf{0.863} &           0.856 \\
table       &    - &  \textbf{0.506} &           0.452 &           0.222 &  \textbf{0.189} &           0.192 &                  - &  \textbf{0.858} &           0.835 \\
telephone   &    - &           0.720 &  \textbf{0.733} &           0.161 &           0.140 &  \textbf{0.128} &                  - &           0.935 &  \textbf{0.936} \\
vessel      &    - &           0.530 &  \textbf{0.544} &  \textbf{0.188} &           0.218 &  \textbf{0.188} &                  - &  \textbf{0.794} &           0.786 \\
\midrule
mean        &    - &  \textbf{0.571} &           0.566 &           0.215 &           0.215 &  \textbf{0.190} &                  - &  \textbf{0.834} &           0.829 \\
\bottomrule
\end{tabular}

==> tables/table_onet_psgn_small.tex <==
\begin{tabular}{lccc}
\toprule
{} &             IoU &   Chamfer-$L_1$ & Normal Consistency \\
\midrule
PSGN        &               - &           0.215 &                  - \\
ONet        &  \textbf{0.571} &           0.215 &     \textbf{0.834} \\
ONet + PSGN &           0.566 &  \textbf{0.190} &              0.829 \\
\bottomrule
\end{tabular}


==> tables/table_pcl2mesh.tex <==
\begin{tabular}{l|cccc|cccc|cccc}
\toprule
{} & \multicolumn{4}{c}{IoU} & \multicolumn{4}{c}{Chamfer-$L_1$} & \multicolumn{4}{c}{Normal Consistency} \\
{} & 3D-R2N2 & PSGN &    DMC &            ONet &       3D-R2N2 &   PSGN &    DMC &            ONet &            3D-R2N2 & PSGN &    DMC &            ONet \\
category    &         &      &        &                 &               &        &        &                 &                    &      &        &                 \\
\midrule
airplane    &   0.464 &    - &  0.570 &  \textbf{0.760} &         0.145 &  0.100 &  0.106 &  \textbf{0.056} &              0.668 &    - &  0.814 &  \textbf{0.897} \\
bench       &   0.441 &    - &  0.536 &  \textbf{0.716} &         0.145 &  0.125 &  0.102 &  \textbf{0.059} &              0.695 &    - &  0.808 &  \textbf{0.878} \\
cabinet     &   0.718 &    - &  0.802 &  \textbf{0.867} &         0.167 &  0.162 &  0.114 &  \textbf{0.073} &              0.790 &    - &  0.887 &  \textbf{0.916} \\
car         &   0.681 &    - &  0.731 &  \textbf{0.835} &         0.197 &  0.130 &  0.166 &  \textbf{0.098} &              0.719 &    - &  0.825 &  \textbf{0.875} \\
chair       &   0.523 &    - &  0.642 &  \textbf{0.736} &         0.181 &  0.165 &  0.121 &  \textbf{0.089} &              0.676 &    - &  0.842 &  \textbf{0.890} \\
display     &   0.603 &    - &  0.753 &  \textbf{0.817} &         0.167 &  0.158 &  0.096 &  \textbf{0.076} &              0.755 &    - &  0.902 &  \textbf{0.926} \\
lamp        &   0.356 &    - &  0.484 &  \textbf{0.566} &         0.231 &  0.202 &  0.170 &  \textbf{0.135} &              0.601 &    - &  0.777 &  \textbf{0.813} \\
loudspeaker &   0.705 &    - &  0.789 &  \textbf{0.828} &         0.200 &  0.201 &  0.151 &  \textbf{0.116} &              0.741 &    - &  0.882 &  \textbf{0.898} \\
rifle       &   0.419 &    - &  0.580 &  \textbf{0.694} &         0.145 &  0.087 &  0.083 &  \textbf{0.060} &              0.707 &    - &  0.780 &  \textbf{0.864} \\
sofa        &   0.704 &    - &  0.800 &  \textbf{0.872} &         0.158 &  0.144 &  0.103 &  \textbf{0.069} &              0.760 &    - &  0.886 &  \textbf{0.928} \\
table       &   0.483 &    - &  0.624 &  \textbf{0.759} &         0.172 &  0.163 &  0.103 &  \textbf{0.071} &              0.742 &    - &  0.874 &  \textbf{0.917} \\
telephone   &   0.699 &    - &  0.848 &  \textbf{0.915} &         0.128 &  0.109 &  0.062 &  \textbf{0.041} &              0.851 &    - &  0.949 &  \textbf{0.970} \\
vessel      &   0.554 &    - &  0.603 &  \textbf{0.748} &         0.163 &  0.126 &  0.150 &  \textbf{0.085} &              0.647 &    - &  0.798 &  \textbf{0.859} \\
\midrule
mean        &   0.565 &    - &  0.674 &  \textbf{0.778} &         0.169 &  0.144 &  0.117 &  \textbf{0.079} &              0.719 &    - &  0.848 &  \textbf{0.895} \\
\bottomrule
\end{tabular}

==> tables/table_pix2mesh_author.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
{} & \multicolumn{3}{c}{IoU} & \multicolumn{3}{c}{Chamfer-$L_1$} & \multicolumn{3}{c}{Normal Consistency} \\
{} & Pix2Mesh (authors) & Pix2Mesh (reimpl.) &            ONet & Pix2Mesh (authors) & Pix2Mesh (reimpl.) &            ONet & Pix2Mesh (authors) & Pix2Mesh (reimpl.) &            ONet \\
category    &                    &                    &                 &                    &                    &                 &                    &                    &                 \\
\midrule
airplane    &              0.400 &              0.420 &  \textbf{0.571} &              0.191 &              0.187 &  \textbf{0.147} &              0.775 &              0.759 &  \textbf{0.840} \\
bench       &              0.272 &              0.323 &  \textbf{0.485} &              0.198 &              0.201 &  \textbf{0.155} &              0.736 &              0.732 &  \textbf{0.813} \\
cabinet     &              0.609 &              0.664 &  \textbf{0.733} &              0.228 &              0.196 &  \textbf{0.167} &              0.828 &              0.834 &  \textbf{0.879} \\
car         &              0.544 &              0.552 &  \textbf{0.737} &              0.190 &              0.180 &  \textbf{0.159} &              0.762 &              0.756 &  \textbf{0.852} \\
chair       &              0.371 &              0.396 &  \textbf{0.501} &              0.270 &              0.265 &  \textbf{0.228} &              0.745 &              0.746 &  \textbf{0.823} \\
display     &              0.440 &     \textbf{0.490} &           0.471 &              0.245 &     \textbf{0.239} &           0.278 &              0.840 &              0.830 &  \textbf{0.854} \\
lamp        &              0.304 &              0.323 &  \textbf{0.371} &              0.315 &     \textbf{0.308} &           0.479 &              0.688 &              0.666 &  \textbf{0.731} \\
loudspeaker &              0.563 &              0.599 &  \textbf{0.647} &              0.306 &     \textbf{0.285} &           0.300 &              0.796 &              0.782 &  \textbf{0.832} \\
rifle       &              0.341 &              0.402 &  \textbf{0.474} &              0.167 &              0.164 &  \textbf{0.141} &              0.715 &              0.718 &  \textbf{0.766} \\
sofa        &              0.544 &              0.613 &  \textbf{0.680} &              0.233 &              0.212 &  \textbf{0.194} &              0.806 &              0.820 &  \textbf{0.863} \\
table       &              0.323 &              0.395 &  \textbf{0.506} &              0.229 &              0.218 &  \textbf{0.189} &              0.785 &              0.784 &  \textbf{0.858} \\
telephone   &              0.625 &              0.661 &  \textbf{0.720} &              0.156 &              0.149 &  \textbf{0.140} &              0.912 &              0.907 &  \textbf{0.935} \\
vessel      &              0.357 &              0.397 &  \textbf{0.530} &              0.221 &     \textbf{0.212} &           0.218 &              0.716 &              0.699 &  \textbf{0.794} \\
\midrule
mean        &              0.438 &              0.480 &  \textbf{0.571} &              0.227 &              0.216 &  \textbf{0.215} &              0.777 &              0.772 &  \textbf{0.834} \\
\bottomrule
\end{tabular}

==> tables/table_pix3d.tex <==
\begin{tabular}{l|ccccc|ccccc|ccccc}
\toprule
{} & \multicolumn{5}{c}{IoU} & \multicolumn{5}{c}{Chamfer-$L_1$} & \multicolumn{5}{c}{Normal Consistency} \\
{} & 3D-R2N2 & PSGN & AtlasNet &   ONet &           ONet+ &       3D-R2N2 &   PSGN &        AtlasNet &   ONet &           ONet+ &            3D-R2N2 & PSGN & AtlasNet &   ONet &           ONet+ \\
category &         &      &          &        &                 &               &        &                 &        &                 &                    &      &          &        &                 \\
\midrule
chair    &   0.146 &    - &        - &  0.224 &  \textbf{0.319} &         2.572 &  0.750 &  \textbf{0.392} &  0.628 &           0.531 &              0.401 &    - &    0.731 &  0.715 &  \textbf{0.747} \\
desk     &   0.170 &    - &        - &  0.268 &  \textbf{0.414} &         1.776 &  0.760 &  \textbf{0.509} &  1.047 &           0.568 &              0.478 &    - &    0.717 &  0.682 &  \textbf{0.780} \\
sofa     &   0.483 &    - &        - &  0.580 &  \textbf{0.699} &         0.537 &  0.592 &  \textbf{0.367} &  0.427 &           0.413 &              0.645 &    - &    0.792 &  0.817 &  \textbf{0.861} \\
table    &   0.137 &    - &        - &  0.204 &  \textbf{0.345} &         2.665 &  0.979 &           0.556 &  1.071 &  \textbf{0.502} &              0.431 &    - &    0.768 &  0.720 &  \textbf{0.809} \\
\midrule
mean     &   0.234 &    - &        - &  0.319 &  \textbf{0.444} &         1.888 &  0.770 &  \textbf{0.456} &  0.793 &           0.504 &              0.489 &    - &    0.752 &  0.733 &  \textbf{0.799} \\
\bottomrule
\end{tabular}

==> tables/table_pix3d_small.tex <==
\begin{tabular}{lccc}
\toprule
{} &             IoU &   Chamfer-$L_1$ & Normal Consistency \\
\midrule
3D-R2N2  &           0.234 &           1.888 &              0.489 \\
PSGN     &               - &           0.770 &                  - \\
AtlasNet &               - &  \textbf{0.456} &              0.752 \\
ONet     &           0.319 &           0.793 &              0.733 \\
ONet+    &  \textbf{0.444} &           0.504 &     \textbf{0.799} \\
\bottomrule
\end{tabular}


==> tables/table_psgn_original.tex <==
\begin{tabular}{l|ccc|ccc|ccc}
\toprule
{} & \multicolumn{3}{c}{Accuracy} & \multicolumn{3}{c}{Completeness} & \multicolumn{3}{c}{Chamfer-$L_1$} \\
{} & PSGN (2 branch) & PSGN (resnet18) &            ONet & PSGN (2 branch) & PSGN (resnet18) &            ONet & PSGN (2 branch) & PSGN (resnet18) &            ONet \\
category    &                 &                 &                 &                 &                 &                 &                 &                 &                 \\
\midrule
airplane    &           0.113 &  \textbf{0.101} &           0.133 &           0.191 &           0.173 &  \textbf{0.161} &           0.152 &  \textbf{0.137} &           0.147 \\
bench       &           0.161 &  \textbf{0.133} &           0.154 &           0.262 &           0.230 &  \textbf{0.156} &           0.212 &           0.181 &  \textbf{0.155} \\
cabinet     &           0.154 &  \textbf{0.138} &           0.150 &           0.307 &           0.291 &  \textbf{0.184} &           0.231 &           0.215 &  \textbf{0.167} \\
car         &           0.126 &           0.117 &  \textbf{0.116} &           0.235 &           0.221 &  \textbf{0.203} &           0.181 &           0.169 &  \textbf{0.159} \\
chair       &           0.233 &  \textbf{0.187} &           0.223 &           0.333 &           0.307 &  \textbf{0.233} &           0.283 &           0.247 &  \textbf{0.228} \\
display     &           0.258 &  \textbf{0.235} &           0.281 &           0.351 &           0.333 &  \textbf{0.275} &           0.304 &           0.284 &  \textbf{0.278} \\
lamp        &           0.301 &  \textbf{0.275} &           0.402 &           0.372 &  \textbf{0.354} &           0.557 &           0.337 &  \textbf{0.314} &           0.479 \\
loudspeaker &           0.253 &  \textbf{0.245} &           0.285 &           0.403 &           0.386 &  \textbf{0.315} &           0.328 &           0.316 &  \textbf{0.300} \\
rifle       &           0.113 &  \textbf{0.110} &           0.148 &           0.159 &           0.158 &  \textbf{0.134} &           0.136 &  \textbf{0.134} &           0.141 \\
sofa        &           0.206 &  \textbf{0.171} &           0.194 &           0.307 &           0.278 &  \textbf{0.195} &           0.257 &           0.224 &  \textbf{0.194} \\
table       &           0.165 &  \textbf{0.152} &           0.189 &           0.307 &           0.293 &  \textbf{0.189} &           0.236 &           0.222 &  \textbf{0.189} \\
telephone   &           0.140 &  \textbf{0.122} &           0.149 &           0.219 &           0.201 &  \textbf{0.130} &           0.179 &           0.161 &  \textbf{0.140} \\
vessel      &           0.186 &  \textbf{0.153} &           0.197 &           0.249 &  \textbf{0.223} &           0.238 &           0.217 &  \textbf{0.188} &           0.218 \\
\midrule
mean        &           0.185 &  \textbf{0.164} &           0.202 &           0.284 &           0.265 &  \textbf{0.228} &           0.235 &  \textbf{0.215} &  \textbf{0.215} \\
\bottomrule
\end{tabular}

==> tables/table_r2n2_original.tex <==
\begin{tabular}{l|ccc|c}
\toprule
{} & \multicolumn{3}{c}{3D-R2N2 (authors)} & 3D-R2N2 (resnet18) \\
{} &            1 view & 3 views &         5 views &             1 view \\
category    &                   &         &                 &                    \\
\midrule
airplane    &             0.513 &   0.549 &           0.561 &     \textbf{0.606} \\
bench       &             0.421 &   0.502 &           0.527 &     \textbf{0.562} \\
cabinet     &             0.716 &   0.763 &  \textbf{0.772} &              0.764 \\
car         &             0.798 &   0.829 &           0.836 &     \textbf{0.846} \\
chair       &             0.466 &   0.533 &  \textbf{0.550} &              0.532 \\
display     &             0.468 &   0.545 &  \textbf{0.565} &              0.528 \\
lamp        &             0.381 &   0.415 &  \textbf{0.421} &              0.389 \\
loudspeaker &             0.662 &   0.708 &  \textbf{0.717} &              0.685 \\
rifle       &             0.544 &   0.593 &  \textbf{0.600} &              0.595 \\
sofa        &             0.628 &   0.690 &  \textbf{0.706} &     \textbf{0.706} \\
table       &             0.513 &   0.564 &  \textbf{0.580} &              0.571 \\
telephone   &             0.661 &   0.732 &  \textbf{0.754} &              0.740 \\
vessel      &             0.513 &   0.596 &  \textbf{0.610} &              0.606 \\
\midrule
mean        &             0.560 &   0.617 &  \textbf{0.631} &              0.625 \\
\bottomrule
\end{tabular}

==> tables/table_voxels2mesh.tex <==
\begin{tabular}{l|cc|cc|cc}
\toprule
{} & \multicolumn{2}{c}{IoU} & \multicolumn{2}{c}{Chamfer-$L_1$} & \multicolumn{2}{c}{Normal Consistency} \\
{} &           Input &            ONet &           Input &            ONet &              Input &            ONet \\
category &                 &                 &                 &                 &                    &                 \\
\midrule
0        &           0.498 &  \textbf{0.722} &           0.127 &  \textbf{0.069} &              0.734 &  \textbf{0.889} \\
1        &           0.504 &  \textbf{0.610} &           0.122 &  \textbf{0.084} &              0.792 &  \textbf{0.854} \\
2        &           0.772 &  \textbf{0.810} &           0.147 &  \textbf{0.112} &              0.896 &  \textbf{0.906} \\
3        &           0.695 &  \textbf{0.807} &           0.188 &  \textbf{0.108} &              0.748 &  \textbf{0.867} \\
4        &           0.622 &  \textbf{0.664} &           0.130 &  \textbf{0.115} &              0.798 &  \textbf{0.873} \\
5        &           0.686 &  \textbf{0.715} &           0.129 &  \textbf{0.117} &              0.878 &  \textbf{0.912} \\
6        &           0.496 &  \textbf{0.511} &  \textbf{0.139} &           0.182 &              0.706 &  \textbf{0.801} \\
7        &  \textbf{0.787} &           0.786 &           0.152 &  \textbf{0.150} &              0.845 &  \textbf{0.888} \\
8        &           0.474 &  \textbf{0.611} &           0.123 &  \textbf{0.080} &              0.768 &  \textbf{0.838} \\
9        &           0.759 &  \textbf{0.802} &           0.129 &  \textbf{0.101} &              0.854 &  \textbf{0.907} \\
10       &           0.582 &  \textbf{0.617} &           0.130 &  \textbf{0.110} &              0.868 &  \textbf{0.894} \\
11       &           0.723 &  \textbf{0.807} &           0.120 &  \textbf{0.080} &              0.891 &  \textbf{0.958} \\
12       &           0.608 &  \textbf{0.679} &           0.135 &  \textbf{0.114} &              0.746 &  \textbf{0.841} \\
\midrule
mean     &           0.631 &  \textbf{0.703} &           0.136 &  \textbf{0.109} &              0.810 &  \textbf{0.879} \\
\bottomrule
\end{tabular}
